DeepObjStyle: Deep Object-based Photo Style Transfer

One of the major challenges of style transfer is the appropriate image features supervision between the output image and the input (style and content) images. An efficient strategy would be to define an object map between the objects of the style and the content images. However, such a mapping is not well established when there are semantic objects of different types and numbers in the style and the content images. It also leads to content mismatch in the style transfer output, which could reduce the visual quality of the results. We propose an object-based style transfer approach, called DeepObjStyle, for the style supervision in the training data-independent framework. DeepObjStyle preserves the semantics of the objects and achieves better style transfer in the challenging scenario when the style and the content images have a mismatch of image features. We also perform style transfer of images containing a word cloud to demonstrate that DeepObjStyle enables an appropriate image features supervision. We validate the results using quantitative comparisons and user studies.

==> deldel <==


    \includegraphics[width=\linewidth]{new_images/Geomatry/in45/tar45_style.jpg}\\
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth]{new_images/Geomatry/in45/blank.jpg}\end{minipage}%
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth]{new_images/Geomatry/in45/blank.jpg}\end{minipage}   \caption{\small  Style} 
\begin{subfigure}[b]{0.132\linewidth}\centering\includegraphics[width=\linewidth]{new_images/Geomatry/in45/box_2_in45.jpg} \\
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=blue 0.1pt 0.1pt]{new_images/Geomatry/in45/crop_1_in45.jpg}\end{minipage}% 
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=red 0.1pt 0.1pt]{new_images/Geomatry/in45/crop_2_in45.jpg}\end{minipage}%
\begin{subfigure}[b]{0.132\linewidth}\centering\includegraphics[width=\linewidth]{new_images/Geomatry/in45/DST_box_2_in45_cSeg_tar45_sSeg.jpg} \\
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=blue 0.1pt 0.1pt]{new_images/Geomatry/in45/DST_crop_2_in45_cSeg_tar45_sSeg.jpg}\end{minipage}%
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=red 0.1pt 0.1pt]{new_images/Geomatry/in45/DST_crop_1_in45_cSeg_tar45_sSeg.jpg}\end{minipage} \caption{\small  DPS  \cite{luan2017deep}} \end{subfigure}\hspace*{1pt}%%
\begin{subfigure}[b]{0.132\linewidth}\centering\includegraphics[width=\linewidth]{new_images/Geomatry/in45/CL_box_2_in45_cSeg_tar45_sSeg.jpg} \\
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=blue 0.1pt 0.1pt]{new_images/Geomatry/in45/CL_crop_2_in45_cSeg_tar45_sSeg.jpg}\end{minipage}%
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=red 0.1pt 0.1pt]{new_images/Geomatry/in45/CL_crop_1_in45_cSeg_tar45_sSeg.jpg}\end{minipage} \caption{\small  CL \cite{mechrez2018contextual}+$\mathcal{L}_m$\cite{luan2017deep}}\end{subfigure}\hspace*{1pt}%%
\begin{subfigure}[b]{0.132\linewidth}\centering\includegraphics[width=\linewidth]{new_images/Geomatry/in45/box_2_q5_WCT2.jpg} \\
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=blue 0.1pt 0.1pt]{new_images/Geomatry/in45/crop_2q5_WCT2.jpg}\end{minipage}%
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=red 0.1pt 0.1pt]{new_images/Geomatry/in45/crop_1q5_WCT2.jpg}\end{minipage}\caption{\small  WCT2 \cite{yoo2019photorealistic}} \end{subfigure}\hspace*{1pt}%%
\begin{subfigure}[b]{0.132\linewidth}\centering\includegraphics[width=\linewidth]{new_images/Geomatry/in45/box_2_in45_tar45_STROTSS.jpg} \\
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=blue 0.1pt 0.1pt]{new_images/Geomatry/in45/crop_2in45_tar45_STROTSS.jpg}\end{minipage}%
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=red 0.1pt 0.1pt]{new_images/Geomatry/in45/crop_1in45_tar45_STROTSS.jpg}\end{minipage}\caption{\small  STROTSS  \cite{kolkin2019style}} \end{subfigure} \hspace*{1pt}%
\begin{subfigure}[b]{0.132\linewidth}\centering\includegraphics[width=\linewidth]{new_images/Geomatry/in45/CLDST_box_2_in45_cSeg_tar45_sSeg.jpg} \\
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=blue 0.1pt 0.1pt]{new_images/Geomatry/in45/CLDST_crop_2_in45_cSeg_tar45_sSeg.jpg}\end{minipage}%
\begin{minipage}{0.49\linewidth}\includegraphics[width=\linewidth, cfbox=red 0.1pt 0.1pt]{new_images/Geomatry/in45/CLDST_crop_1_in45_cSeg_tar45_sSeg.jpg}\end{minipage} \caption{\small  DeepObjStyle}\end{subfigure}} \end{center}
\begin{subfigure}{0.145\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleDiffusion/tar7_style.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth]{new_images/StyleDiffusion/blank.jpg}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth]{new_images/StyleDiffusion/blank.jpg}\end{subfigure} \caption{Style $S$}\end{center} \end{subfigure}
\begin{subfigure}{0.145\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleDiffusion/box_2_content_in1_content.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_2content_in1_content.jpg}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_1content_in1_content.jpg}\end{subfigure} \caption{Content $C$}\end{center} \end{subfigure}
\begin{subfigure}{0.145\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleDiffusion/box_2_neural_style_in1_cSeg_tar7_sSeg.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_2neural_style_in1_cSeg_tar7_sSeg.jpg} \end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_1neural_style_in1_cSeg_tar7_sSeg.jpg}\end{subfigure}\caption{Neural style\cite{gatys2016image} }\end{center} \end{subfigure}
\begin{subfigure}{0.145\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleDiffusion/box_2_DST_in1_cSeg_tar7_sSeg.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_2DST_in1_cSeg_tar7_sSeg.jpg}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_1DST_in1_cSeg_tar7_sSeg.jpg}\end{subfigure}\caption{DPS \cite{luan2017deep} }\end{center} \end{subfigure}
\begin{subfigure}{0.145\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleDiffusion/box_2_q11_WCT2.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_2q11_WCT2.jpg}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_1q11_WCT2.jpg}\end{subfigure}\caption{WCT2 \cite{yoo2019photorealistic} }\end{center} \end{subfigure}
\begin{subfigure}{0.145\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleDiffusion/box_2_in1_tar7_STROTSS.jpg} \\
\begin{subfigure}{0.49\textwidth}\includegraphics[width=\linewidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_2_in1_tar7_STROTSS.jpg}\end{subfigure}%
\begin{subfigure}{0.49\textwidth}\includegraphics[width=\linewidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_1_in1_tar7_STROTSS.jpg}\end{subfigure} \caption{STROTSS  \cite{kolkin2019style}}\end{center} \end{subfigure}  \hspace*{0.1pt}%
\begin{subfigure}{0.145\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleDiffusion/box_2_content_more_in1_cSeg_tar7_sSeg_deepObjStyle.png} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_2content_more_in1_cSeg_tar7_sSeg_deepObjStyle.png}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleDiffusion/crop_1content_more_in1_cSeg_tar7_sSeg_deepObjStyle.png}\end{subfigure} \caption{DeepObjStyle} 
\begin{subfigure}{0.135\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleUtilization/tar32_style.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth]{new_images/StyleUtilization/blank.jpg}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth]{new_images/StyleUtilization/blank.jpg}\end{subfigure} \caption{Style $S$}\end{center} \end{subfigure}
\begin{subfigure}{0.135\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleUtilization/box_2_content_in14_content.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleUtilization/crop_2content_in14_content.jpg}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleUtilization/crop_1content_in14_content.jpg}\end{subfigure}\caption{Content $C$}\end{center} \end{subfigure}
\begin{subfigure}{0.135\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleUtilization/box_2_DST_in14_cSeg_tar32_sSeg.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleUtilization/crop_2DST_in14_cSeg_tar32_sSeg.jpg}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleUtilization/crop_1DST_in14_cSeg_tar32_sSeg.jpg}\end{subfigure}\caption{DPS \cite{luan2017deep}}\end{center} \end{subfigure}
\begin{subfigure}{0.135\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleUtilization/box_2_DST_plus_style_more_in14_cSeg_tar32_sSeg.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleUtilization/crop_2DST_plus_style_more_in14_cSeg_tar32_sSeg.jpg}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleUtilization/crop_1DST_plus_style_more_in14_cSeg_tar32_sSeg.jpg}\end{subfigure} \caption{DPS$^+$}\end{center} \end{subfigure}
\begin{subfigure}{0.135\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleUtilization/box_2_q12_WCT2.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleUtilization/crop_2q12_WCT2.jpg}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleUtilization/crop_1q12_WCT2.jpg}\end{subfigure} \caption{WCT2 \cite{yoo2019photorealistic} }\end{center} \end{subfigure}
\begin{subfigure}{0.135\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleUtilization/box_2_in14_tar32_STROTSS.jpg} \\
\begin{subfigure}{0.49\textwidth}\includegraphics[width=\linewidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleUtilization/crop_2in14_tar32_STROTSS.jpg}\end{subfigure}%
\begin{subfigure}{0.49\textwidth}\includegraphics[width=\linewidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleUtilization/crop_1in14_tar32_STROTSS.jpg}\end{subfigure}  \caption{STROTSS  \cite{kolkin2019style}}\end{center} \end{subfigure} %\hspace*{0.01pt} %
\begin{subfigure}{0.135\linewidth}\begin{center}\includegraphics[width=\textwidth]{new_images/StyleUtilization/box_2_style_more_in14_cSeg_tar32_sSeg.jpg} \\
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=red 0.1pt 0.1pt]{new_images/StyleUtilization/crop_2style_more_in14_cSeg_tar32_sSeg.jpg}\end{subfigure}%
\begin{subfigure}{0.5\textwidth}\includegraphics[width=\textwidth, cfbox=blue 0.1pt 0.1pt]{new_images/StyleUtilization/crop_1style_more_in14_cSeg_tar32_sSeg.jpg}\end{subfigure}\caption{DeepObjStyle}\end{center} \end{subfigure}} \end{center}


\begin{subfigure}[b]{0.3\linewidth} \includegraphics[width=\linewidth]{Question/q8/l4_content_style.png} \caption{\small  Content \& Style} \end{subfigure}\hspace*{1pt} %%
\begin{subfigure}[b]{0.3\linewidth} \includegraphics[width=\linewidth]{Question/q8/STROTSS_l4_cSeg_d4_sSeg.png}\caption{\small  STROTSS \cite{kolkin2019style}}\end{subfigure}\hspace*{1pt} %%
\begin{subfigure}[b]{0.3\linewidth} \includegraphics[width=\linewidth]{Question/q8/CLDST_l4_cSeg_d4_sSeg.png}\caption{\small  DeepObjStyle}\end{subfigure}\vspace*{-0.15cm}


